Sphere Window: Challenges and Opportunities of 360{\deg} Video in Collaborative Design Workshops

The increased ubiquity of 360{\deg} video presents a unique opportunity for designers to deeply engage with the world of users by capturing the complete visual context. However, the opportunities and challenges 360{\deg} video introduces for video design ethnography is unclear. This study investigates this gap through 16 workshops in which experienced designers engaged with 360{\deg} video. Our analysis shows that while 360{\deg} video enhances designers' ability to explore and understand user contexts, it also complicates the process of sharing insights. To address this challenge, we present two opportunities to support the use of 360{\deg} video by designers - the creation of designerly 360{\deg} video annotation tools, and 360{\deg} ``screenshots'' - in order to enable designers to leverage the complete context of 360{\deg} video for user research.

==> content/design_directions.tex <==
Using the behaviors, themes, and ideation output presented in Section~\ref{results}, we present a number of features for future 360° video tools for designers to use in the early stage of the design process. Based on these features, we derived three example design directions based on \hl{analysis of the ideation sessions during the workshops. Where possible, we refer to works that explore these interactions, but as noted in Section~{\ref{hci_360}}, these works are not focused on how designers use 360° video, and thus the interactions they discuss need to be re-evaluated for the workflow of designers conducting user research with video.}
\begin{figure*}[hb]
    \centering
    \subfloat[A bespoke 360° video analysis tool could allow asymetric collaboration, where one viewer uses a VR headset while the other uses a laptop to annotate the same 360° video]{\label{fig:parity}\includegraphics[width=0.35\textwidth]{content/images/design-directions/design directions-03.png}\Description{A cartoonish representatin of two people viewing the same 360 video. One is wearing a VR headset and the other is using a laptop. Above them there is a single frame of 360 video showing both their viewpoints.}}
    \qquad
    \subfloat[An example of a 360° specific screenshot with, an overview of the full frame, a QR code to pull up the annotation on a computer, and two sub-screenshots that show an action happening ``across the frame'']{\label{fig:future-screenshot}\includegraphics[width=0.35\textwidth]{content/images/design-directions/design directions-01.png}\Description{A piece of paper that shows a rectangular projection of a frame of 360 video with two green rectangles highlighting two areas. Below that are the two areas in greater detail with a line connecting them, showing that designers can create connections between them. Finally on the bottom is a QR code and some placeholder text to show that the screenshot can link back to a 360 video.}}
    \caption{Illustrating the two design directions for future tools to support 360° video design ethnography.}
    \label{fig:design-directions}
\end{figure*}
\begin{enumerate}[label= DD \arabic*]
    \item \label{360-first-viewer} \textbf{Designerly 360° viewer:} Designers could benefit from a 360° video specific analysis tool that allows viewers to label screenshots in-situ~\footnote{Rather than first watching the video, and then annotating screenshots--a limitation of the workflow of current tools.} and have a library of existing labels and annotations. Since these annotations are recorded by the viewing software, it would be possible to share the annotations and viewpoints of others, forming a better shared understanding of the content~\cite{nguyen_collavr_2017}. This asynchronous collaboration helps balance the benefits of collaboratively annotating 360° videos~\cite{vatanen_experiences_2022} with the flexibility of being able to view individually.\\
    The tool should work on laptops, phones, and VR-headsets so that viewers can switch between them seamlessly; both for their comfort (\ref{different-tools}) and to take advantage of the different viewpoint of the tools (\ref{immersion-usability-spectrum}). This enables asymmetric annotation, where one viewer uses the more immersive VR headset while another uses the more ``forensic'' view afforded by the laptop. This notion of asymmetrical interaction has been used to help annotate virtual environments~\cite{thoravi_kumaravel_transceivr_2020} or creating storyboards for VR stories~\cite{henrikson_multi-device_2016} as it enables one person to remain immersed in a VR headset while the other does more detailed tasks (e.g., sketching, typing, or highlighting specific areas). Lastly, the tool presents an opportunity to use techniques to reduce FOMO, such as adding panoramic thumbnails~\cite{yamaguchi_now_2021}, picture-in-picture overlays~\cite{lin_outside-_2017}, or by shifting the \hl{viewpoint of the video}~\cite{tanaka_attracting_2015,aitamurto_fomo_2021,gugenheimer_swivrchair_2016}.

    \item \label{360-first-screenshots} \textbf{Refining Screenshots for Sharing 360° Video:} To enhance how designers use the sharing of flat, physical screenshots during collaborative workshops with the contextual richness of 360° videos, we propose the creation of ``360° screenshots. These screenshots could include additional information about the 360° frame in which they were taken by including a 360° thumbnail, as well as an overview of the perspective and timestamp. A QR code linking to this video would drastically reduce the hassle of switching to the 360° video and allow designers to share not only the full 360° video, but also the motion, sound, and insights that led up to the annotation.\\
    More specifically, an annotation tool should support the creation of ``composite'' or ``scattered'' multi-screenshots (\ref{beyond-normal-screenshot}) so that designers can document and share insights based on multiple parts of a single frame of 360° video. Further exploration of different 360° specific screenshots (e.g., different types of projections, overlays, or multi-screenshots) could lead to a new visual language for discussing and sharing 360° videos, similar to the manga-inspired methods for sharing videos explored by~\citet{uchihashi_video_1999}.
\end{enumerate}
